An $O(n$)-Algorithm for the Higher-Order Kinematics and Inverse Dynamics of Serial Manipulators using Spatial Representation of Twists

Optimal control in general, and flatness-based control in particular, of robotic arms necessitate to compute the first and second time derivatives of the joint torques/forces required to achieve a desired motion. In view of the required computational efficiency, recursive $O(n)$-algorithms were proposed to this end. Aiming at compact yet efficient formulations, a Lie group formulation was recently proposed, making use of body-fixed and hybrid representation of twists and wrenches. In this paper a formulation is introduced using the spatial representation. The second-order inverse dynamics algorithm is accompanied by a fourth-order forward and inverse kinematics algorithm. An advantage of all Lie group formulations is that they can be parameterized in terms of vectorial quantities that are readily available. The method is demonstrated for the 7 DOF Franka Emika Panda robot.

==> Algorithm1.tex <==
%TCIDATA{Version=5.50.0.2960}
%TCIDATA{LaTeXparent=0,0,HighOrderInverseDyn.tex}
\begin{figure}[ht]
\begin{tabular}{l}
\textbf{Algorithm 1: }%
%TCIMACRO{\TeXButton{red}{\color{red}}}%
%BeginExpansion
\color{red}%
%EndExpansion
\textbf{4th-Order Forward Kinematics Recursion}%
%TCIMACRO{\TeXButton{black}{\color{black}} }%
%BeginExpansion
\color{black}
%EndExpansion
\\ \hline
\textbf{Input:} $\mathbf{q},\dot{\mathbf{q}},\ddot{\mathbf{q}},\dddot{%
\mathbf{q}},\ddot{\ddot{\mathbf{q}}}$, and $\mathbf{Y}_{i},i=1,\ldots ,n$ \\ 
For $i=1,\ldots ,n$ do \\ 
\begin{tabular}{rll}
$f_{i}%
%TCIMACRO{\TeXButton{-2ex}{\hspace{-2ex}}}%
%BeginExpansion
\hspace{-2ex}%
%EndExpansion
$ & $=%
%TCIMACRO{\TeXButton{-2ex}{\hspace{-2ex}}}%
%BeginExpansion
\hspace{-2ex}%
%EndExpansion
$ & $f_{i-1}\exp (\mathbf{Y}_{i}q_{i})$ \ \ \ \ \ \ \ \ \ Position kinematics
\\ 
$\mathbf{C}_{i}%
%TCIMACRO{\TeXButton{-2ex}{\hspace{-2ex}}}%
%BeginExpansion
\hspace{-2ex}%
%EndExpansion
$ & $=%
%TCIMACRO{\TeXButton{-2ex}{\hspace{-2ex}}}%
%BeginExpansion
\hspace{-2ex}%
%EndExpansion
$ & $f_{i}\mathbf{A}_{i}$ \\ 
$\mathbf{S}_{i}%
%TCIMACRO{\TeXButton{-2ex}{\hspace{-2ex}}}%
%BeginExpansion
\hspace{-2ex}%
%EndExpansion
$ & $=%
%TCIMACRO{\TeXButton{-2ex}{\hspace{-2ex}}}%
%BeginExpansion
\hspace{-2ex}%
%EndExpansion
$ & $\mathbf{Ad}_{f_{i}\left( \mathbf{q}\right) }\mathbf{Y}_{i}\ \ \ \ \ \ \
\ \ \ \ \ \ \ \ $Higher-order kinematics \\ 
$\mathbf{V}_{i}^{\text{\textrm{s}}}%
%TCIMACRO{\TeXButton{-2ex}{\hspace{-2ex}}}%
%BeginExpansion
\hspace{-2ex}%
%EndExpansion
$ & $=%
%TCIMACRO{\TeXButton{-2ex}{\hspace{-2ex}}}%
%BeginExpansion
\hspace{-2ex}%
%EndExpansion
$ & $\mathbf{V}_{i-1}^{\text{\textrm{s}}}+\mathbf{S}_{i}\dot{q}_{i}$ \\ 
$\dot{\mathbf{S}}_{i}%
%TCIMACRO{\TeXButton{-2ex}{\hspace{-2ex}}}%
%BeginExpansion
\hspace{-2ex}%
%EndExpansion
$ & $=%
%TCIMACRO{\TeXButton{-2ex}{\hspace{-2ex}}}%
%BeginExpansion
\hspace{-2ex}%
%EndExpansion
$ & $\mathbf{ad}_{\mathbf{V}_{i}^{\text{\textrm{s}}}}\mathbf{S}_{i}$ \\ 
$\dot{\mathbf{V}}_{i}^{\text{\textrm{s}}}%
%TCIMACRO{\TeXButton{-2ex}{\hspace{-2ex}}}%
%BeginExpansion
\hspace{-2ex}%
%EndExpansion
$ & $=%
%TCIMACRO{\TeXButton{-2ex}{\hspace{-2ex}}}%
%BeginExpansion
\hspace{-2ex}%
%EndExpansion
$ & $\dot{\mathbf{V}}_{i-1}^{\text{\textrm{s}}}+\mathbf{S}_{i}\ddot{q}_{i}+%
\dot{\mathbf{S}}_{i}\dot{q}_{i}$ \\ 
$\ddot{\mathbf{S}}_{i}%
%TCIMACRO{\TeXButton{-2ex}{\hspace{-2ex}}}%
%BeginExpansion
\hspace{-2ex}%
%EndExpansion
$ & $=%
%TCIMACRO{\TeXButton{-2ex}{\hspace{-2ex}}}%
%BeginExpansion
\hspace{-2ex}%
%EndExpansion
$ & $%
%TCIMACRO{\TeXButton{big}{\big}}%
%BeginExpansion
\big%
%EndExpansion
(\mathbf{ad}_{\dot{\mathbf{V}}_{i}^{\text{\textrm{s}}}}+\mathbf{ad}_{\mathbf{%
V}_{i}^{\text{\textrm{s}}}}^{2}%
%TCIMACRO{\TeXButton{big}{\big}}%
%BeginExpansion
\big%
%EndExpansion
)\mathbf{S}_{i}$ \\ 
$\ddot{\mathbf{V}}_{i}^{\text{\textrm{s}}}%
%TCIMACRO{\TeXButton{-2ex}{\hspace{-2ex}}}%
%BeginExpansion
\hspace{-2ex}%
%EndExpansion
$ & $=%
%TCIMACRO{\TeXButton{-2ex}{\hspace{-2ex}}}%
%BeginExpansion
\hspace{-2ex}%
%EndExpansion
$ & $\ddot{\mathbf{V}}_{i-1}^{\text{\textrm{s}}}+\mathbf{S}_{i}\dddot{q}%
_{i}+2\dot{\mathbf{S}}_{i}\ddot{q}_{i}+\ddot{\mathbf{S}}_{i}\dot{q}_{i}$ \\ 
$\dddot{\mathbf{S}}_{i}%
%TCIMACRO{\TeXButton{-2ex}{\hspace{-2ex}}}%
%BeginExpansion
\hspace{-2ex}%
%EndExpansion
$ & $=%
%TCIMACRO{\TeXButton{-2ex}{\hspace{-2ex}}}%
%BeginExpansion
\hspace{-2ex}%
%EndExpansion
$ & $%
%TCIMACRO{\TeXButton{big}{\big}}%
%BeginExpansion
\big%
%EndExpansion
(\mathbf{ad}_{\ddot{\mathbf{V}}_{i}^{\text{\textrm{s}}}}+2\mathbf{ad}_{\dot{%
\mathbf{V}}_{i}^{\text{\textrm{s}}}}\mathbf{ad}_{\mathbf{V}_{i}^{\text{%
\textrm{s}}}}+\mathbf{ad}_{\mathbf{V}_{i}^{\text{\textrm{s}}}}\mathbf{ad}_{%
\dot{\mathbf{V}}_{i}^{\text{\textrm{s}}}}+\mathbf{ad}_{\mathbf{V}_{i}^{\text{%
\textrm{s}}}}^{3}%
%TCIMACRO{\TeXButton{big}{\big}}%
%BeginExpansion
\big%
%EndExpansion
)\mathbf{S}_{i}$ \\ 
$\dddot{\mathbf{V}}_{i}^{\text{\textrm{s}}}%
%TCIMACRO{\TeXButton{-2ex}{\hspace{-2ex}}}%
%BeginExpansion
\hspace{-2ex}%
%EndExpansion
$ & $=%
%TCIMACRO{\TeXButton{-2ex}{\hspace{-2ex}}}%
%BeginExpansion
\hspace{-2ex}%
%EndExpansion
$ & $\dddot{\mathbf{V}}_{i-1}^{\text{\textrm{s}}}+\mathbf{S}_{i}\ddot{\ddot{q%
}}_{i}+3\dot{\mathbf{S}}_{i}\dddot{q}_{i}+3\ddot{\mathbf{S}}_{i}\ddot{q}_{i}+%
\dddot{\mathbf{S}}_{i}\dot{q}_{i}$%
\end{tabular}
\\ 
End \\ 
\textbf{Output:} $\mathbf{V}_{i}^{\text{\textrm{s}}},\dot{\mathbf{V}}_{i}^{%
\text{\textrm{s}}},\ddot{\mathbf{V}}_{i}^{\text{\textrm{s}}},\dddot{\mathbf{V%
}}_{i}^{\text{\textrm{s}}}$ and $\mathbf{S}_{i},\dot{\mathbf{S}}_{i},\ddot{%
\mathbf{S}}_{i},\dddot{\mathbf{S}}_{i}$ \\ \hline
\end{tabular}%
\vspace{-3ex}
\end{figure}

==> Algorithm2.tex <==
%TCIDATA{Version=5.50.0.2960}
%TCIDATA{LaTeXparent=0,0,HighOrderInverseDyn.tex}
                      

\begin{tabular}{l}
\textbf{Algorithm 2: } \\ 
\textbf{Combined inverse and forward kinematics recursion} \\ \hline
\textbf{Input:} $\mathbf{q},\mathbf{V}_{\mathrm{E}}^{\text{s}},\dot{\mathbf{V%
}}_{\mathrm{E}}^{\text{s}},\ddot{\mathbf{V}}_{\mathrm{E}}^{\text{s}},\dddot{%
\mathbf{V}}_{\mathrm{E}}^{\text{s}}$, and $\mathbf{Y}_{i},i=1,\ldots ,n$ \\ 
\textbf{1)} \ Configurations, joint screws (EE-Jacobian): \\ 
%TCIMACRO{\TeXButton{9ex}{\hspace{9ex}}}%
%BeginExpansion
\hspace{9ex}%
%EndExpansion
\begin{tabular}{l}
For $i=1,\ldots ,n$ do \\ 
%TCIMACRO{\TeXButton{2ex}{\hspace{2ex}}}%
%BeginExpansion
\hspace{2ex}%
%EndExpansion
$f_{i}=f_{i-1}\exp (\mathbf{Y}_{i}q_{i})$ \\ 
%TCIMACRO{\TeXButton{2ex}{\hspace{2ex}}}%
%BeginExpansion
\hspace{2ex}%
%EndExpansion
$\mathbf{C}_{i}=f_{i}\mathbf{A}_{i}$ \\ 
%TCIMACRO{\TeXButton{2ex}{\hspace{2ex}}}%
%BeginExpansion
\hspace{2ex}%
%EndExpansion
$\mathbf{S}_{i}=\mathbf{Ad}_{f_{i}\left( \mathbf{q}\right) }\mathbf{Y}_{i}$
\\ 
End%
\end{tabular}
\\ 
\textbf{2.a)} \ 1st-order inverse kinematics of manipulator: \\ 
%TCIMACRO{\TeXButton{10ex}{\hspace{10ex}}}%
%BeginExpansion
\hspace{10ex}%
%EndExpansion
$\dot{\mathbf{q}}=\mathbf{J}^{-1}\mathbf{V}_{\mathrm{E}}^{\text{s}}$ \\ 
\textbf{2.b)} \ 1st-order forward kinematics of robot mechanism: \\ 
%TCIMACRO{\TeXButton{9ex}{\hspace{9ex}}}%
%BeginExpansion
\hspace{9ex}%
%EndExpansion
\begin{tabular}{l}
For $i=1,\ldots ,n-1$ do \\ 
%TCIMACRO{\TeXButton{2ex}{\hspace{2ex}}}%
%BeginExpansion
\hspace{2ex}%
%EndExpansion
$\mathbf{V}_{i}^{\text{s}}=\mathbf{V}_{i-1}^{\text{s}}+\mathbf{S}_{i}\dot{q}%
_{i}$ \\ 
%TCIMACRO{\TeXButton{2ex}{\hspace{2ex}}}%
%BeginExpansion
\hspace{2ex}%
%EndExpansion
$~\dot{\mathbf{S}}_{i}=\mathbf{ad}_{\mathbf{V}_{i}^{\text{s}}}\mathbf{S}_{i}$
\\ 
End%
\end{tabular}
\\ 
\textbf{3.a)} \ 2nd-order inverse kinematics of manipulator: \\ 
%TCIMACRO{\TeXButton{10ex}{\hspace{10ex}}}%
%BeginExpansion
\hspace{10ex}%
%EndExpansion
$\ddot{\mathbf{q}}=\mathbf{J}^{-1}%
%TCIMACRO{\TeXButton{Big}{\Big}}%
%BeginExpansion
\Big%
%EndExpansion
(\dot{\mathbf{V}}_{\mathrm{E}}^{\text{s}}-\sum_{i\leq n}\dot{\mathbf{S}}_{i}%
\dot{q}_{i}%
%TCIMACRO{\TeXButton{Big}{\Big}}%
%BeginExpansion
\Big%
%EndExpansion
)$ \\ 
\textbf{3.b)} \ 2nd-order forward kinematics of robot mechanism: \\ 
%TCIMACRO{\TeXButton{9ex}{\hspace{9ex}}}%
%BeginExpansion
\hspace{9ex}%
%EndExpansion
\begin{tabular}{l}
For $i=1,\ldots ,n-1$ do \\ 
%TCIMACRO{\TeXButton{2ex}{\hspace{2ex}}}%
%BeginExpansion
\hspace{2ex}%
%EndExpansion
\begin{tabular}{rl}
$\dot{\mathbf{V}}_{i}^{\text{s}}=%
%TCIMACRO{\TeXButton{-2ex}{\hspace{-2ex}}}%
%BeginExpansion
\hspace{-2ex}%
%EndExpansion
$ & $\mathbf{V}_{i-1}^{\text{s}}+\mathbf{S}_{i}\ddot{q}_{i}+\dot{\mathbf{S}}%
_{i}\dot{q}_{i}$ \\ 
$\ddot{\mathbf{S}}_{i}=%
%TCIMACRO{\TeXButton{-2ex}{\hspace{-2ex}}}%
%BeginExpansion
\hspace{-2ex}%
%EndExpansion
$ & $%
%TCIMACRO{\TeXButton{big}{\big}}%
%BeginExpansion
\big%
%EndExpansion
(\mathbf{ad}_{\dot{\mathbf{V}}_{i}^{\text{s}}}+\mathbf{ad}_{\mathbf{V}_{i}^{%
\text{s}}}^{2}%
%TCIMACRO{\TeXButton{big}{\big}}%
%BeginExpansion
\big%
%EndExpansion
)\mathbf{S}_{i}$%
\end{tabular}
\\ 
End%
\end{tabular}
\\ 
\textbf{4.a)} \ 3rd-order inverse kinematics of manipulator: \\ 
%TCIMACRO{\TeXButton{10ex}{\hspace{10ex}}}%
%BeginExpansion
\hspace{10ex}%
%EndExpansion
$\dddot{\mathbf{q}}=\mathbf{J}^{-1}%
%TCIMACRO{\TeXButton{Big}{\Big}}%
%BeginExpansion
\Big%
%EndExpansion
(\ddot{\mathbf{V}}_{\mathrm{E}}^{\text{s}}-\sum_{i\leq n}(2\dot{\mathbf{S}}%
_{i}\ddot{q}_{i}+\ddot{\mathbf{S}}_{i}\dot{q}_{i})%
%TCIMACRO{\TeXButton{Big}{\Big}}%
%BeginExpansion
\Big%
%EndExpansion
)$ \\ 
\textbf{4.b)} \ 3rd-order forward kinematics of robot mechanism: \\ 
%TCIMACRO{\TeXButton{1ex}{\hspace{1ex}}}%
%BeginExpansion
\hspace{1ex}%
%EndExpansion
\begin{tabular}{l}
For $i=1,\ldots ,n-1$ do \\ 
%TCIMACRO{\TeXButton{1ex}{\hspace{1ex}}}%
%BeginExpansion
\hspace{1ex}%
%EndExpansion
\begin{tabular}{rl}
$\ddot{\mathbf{V}}_{i}^{\text{s}}=%
%TCIMACRO{\TeXButton{-2ex}{\hspace{-2ex}}}%
%BeginExpansion
\hspace{-2ex}%
%EndExpansion
$ & $\ddot{\mathbf{V}}_{i-1}^{\text{s}}+\mathbf{S}_{i}\dddot{q}_{i}+2\dot{%
\mathbf{S}}_{i}\ddot{q}_{i}+\ddot{\mathbf{S}}_{i}\dot{q}_{i}$ \\ 
$\dddot{\mathbf{S}}_{i}=%
%TCIMACRO{\TeXButton{-2ex}{\hspace{-2ex}}}%
%BeginExpansion
\hspace{-2ex}%
%EndExpansion
$ & $%
%TCIMACRO{\TeXButton{big}{\big}}%
%BeginExpansion
\big%
%EndExpansion
(\mathbf{ad}_{\ddot{\mathbf{V}}_{i}^{\text{s}}}+2\mathbf{ad}_{\dot{\mathbf{V}%
}_{i}^{\text{s}}}\mathbf{ad}_{\mathbf{V}_{i}^{\text{s}}}+\mathbf{ad}_{%
\mathbf{V}_{i}^{\text{s}}}\mathbf{ad}_{\dot{\mathbf{V}}_{i}^{\text{s}}}+%
\mathbf{ad}_{\mathbf{V}_{i}^{\text{s}}}^{3}%
%TCIMACRO{\TeXButton{big}{\big}}%
%BeginExpansion
\big%
%EndExpansion
)\mathbf{S}_{i}$%
\end{tabular}
\\ 
End%
\end{tabular}
\\ 
\textbf{5.a)} \ 4th-order inverse kinematics of manipulator: \\ 
$\ddot{\ddot{\mathbf{q}}}=\mathbf{J}^{-1}%
%TCIMACRO{\TeXButton{Big}{\Big}}%
%BeginExpansion
\Big%
%EndExpansion
(\dddot{\mathbf{V}}_{n}^{\text{s}}-\sum_{i\leq n}(\dot{\mathbf{S}}_{i}\dddot{%
q}_{i}+3\ddot{\mathbf{S}}_{i}\ddot{q}_{i}+\dddot{\mathbf{S}}_{i}\dot{q}_{i})%
%TCIMACRO{\TeXButton{Big}{\Big}}%
%BeginExpansion
\Big%
%EndExpansion
)$ \\ 
%TCIMACRO{\TeXButton{4ex}{\hspace{4ex}} }%
%BeginExpansion
\hspace{4ex}
%EndExpansion
\\ 
\textbf{5.b)} \ 4th-order forward kinematics of robot mechanism: \\ 
\begin{tabular}{l}
For $i=1,\ldots ,n-1$ do \\ 
%TCIMACRO{\TeXButton{2ex}{\hspace{2ex}}}%
%BeginExpansion
\hspace{2ex}%
%EndExpansion
$\dddot{\mathbf{V}}_{i}^{\text{s}}=\dddot{\mathbf{V}}_{i-1}^{\text{s}}+%
\mathbf{S}_{i}\ddot{\ddot{q}}_{i}+3\dot{\mathbf{S}}_{i}\dddot{q}_{i}+3\ddot{%
\mathbf{S}}_{i}\ddot{q}_{i}+\dddot{\mathbf{S}}_{i}\dot{q}_{i}$ \\ 
End%
\end{tabular}
\\ 
\textbf{Output:} $\dot{\mathbf{q}},\ddot{\mathbf{q}},\dddot{\mathbf{q}},%
\ddot{\ddot{\mathbf{q}}}$, $\dot{\mathbf{S}}_{i},\ddot{\mathbf{S}}_{i},%
\dddot{\mathbf{S}}_{i}$, $\mathbf{V}_{i}^{\text{s}},\dot{\mathbf{V}}_{i}^{%
\text{s}},\ddot{\mathbf{V}}_{i}^{\text{s}},\dddot{\mathbf{V}}_{i}^{\text{s}}$%
, $\mathbf{J}\left( \mathbf{q}\right) $ \\ \hline
\end{tabular}


==> Algorithm2tmp.tex <==
%TCIDATA{Version=5.50.0.2960}
%TCIDATA{LaTeXparent=0,0,HighOrderInverseDyn.tex}
                      

\begin{figure}[ht]
\begin{tabular}{l}
\textbf{Algorithm 2: } \\ 
\textbf{Combined inverse and forward kinematics recursion} \\ \hline
\textbf{Input:} $\mathbf{q},\mathbf{V}_{\mathrm{E}}^{\text{s}},\dot{\mathbf{V%
}}_{\mathrm{E}}^{\text{s}},\ddot{\mathbf{V}}_{\mathrm{E}}^{\text{s}},\dddot{%
\mathbf{V}}_{\mathrm{E}}^{\text{s}}$, and $\mathbf{Y}_{i},i=1,\ldots ,n$ \\ 
\textbf{1)} \ Configurations, joint screws (EE-Jacobian): \\ 
%TCIMACRO{\TeXButton{9ex}{\hspace{9ex}}}%
%BeginExpansion
\hspace{9ex}%
%EndExpansion
\begin{tabular}{l}
For $i=1,\ldots ,n$ do \\ 
%TCIMACRO{\TeXButton{2ex}{\hspace{2ex}}}%
%BeginExpansion
\hspace{2ex}%
%EndExpansion
$f_{i}=f_{i-1}\exp (\mathbf{Y}_{i}q_{i})$ \\ 
%TCIMACRO{\TeXButton{2ex}{\hspace{2ex}}}%
%BeginExpansion
\hspace{2ex}%
%EndExpansion
$\mathbf{C}_{i}=f_{i}\mathbf{A}_{i}$ \\ 
%TCIMACRO{\TeXButton{2ex}{\hspace{2ex}}}%
%BeginExpansion
\hspace{2ex}%
%EndExpansion
$\mathbf{S}_{i}=\mathbf{Ad}_{f_{i}\left( \mathbf{q}\right) }\mathbf{Y}_{i}$
\\ 
End%
\end{tabular}
\\ 
\textbf{2.a)} \ 1st-order inverse kinematics of manipulator: \\ 
%TCIMACRO{\TeXButton{10ex}{\hspace{10ex}}}%
%BeginExpansion
\hspace{10ex}%
%EndExpansion
$\dot{\mathbf{q}}=\mathbf{J}^{-1}\mathbf{V}_{\mathrm{E}}^{\text{s}}$ \\ 
\textbf{2.b)} \ 1st-order forward kinematics of robot mechanism: \\ 
%TCIMACRO{\TeXButton{9ex}{\hspace{9ex}}}%
%BeginExpansion
\hspace{9ex}%
%EndExpansion
\begin{tabular}{l}
For $i=1,\ldots ,n-1$ do \\ 
%TCIMACRO{\TeXButton{2ex}{\hspace{2ex}}}%
%BeginExpansion
\hspace{2ex}%
%EndExpansion
$\mathbf{V}_{i}^{\text{s}}=\mathbf{V}_{i-1}^{\text{s}}+\mathbf{S}_{i}\dot{q}%
_{i}$ \\ 
%TCIMACRO{\TeXButton{2ex}{\hspace{2ex}}}%
%BeginExpansion
\hspace{2ex}%
%EndExpansion
$~\dot{\mathbf{S}}_{i}=\mathbf{ad}_{\mathbf{V}_{i}^{\text{s}}}\mathbf{S}_{i}$
\\ 
End%
\end{tabular}
\\ 
\textbf{3.a)} \ 2nd-order inverse kinematics of manipulator: \\ 
%TCIMACRO{\TeXButton{10ex}{\hspace{10ex}}}%
%BeginExpansion
\hspace{10ex}%
%EndExpansion
$\ddot{\mathbf{q}}=\mathbf{J}^{-1}%
%TCIMACRO{\TeXButton{Big}{\Big}}%
%BeginExpansion
\Big%
%EndExpansion
(\dot{\mathbf{V}}_{\mathrm{E}}^{\text{s}}-\sum_{i\leq n}\dot{\mathbf{S}}_{i}%
\dot{q}_{i}%
%TCIMACRO{\TeXButton{Big}{\Big}}%
%BeginExpansion
\Big%
%EndExpansion
)$ \\ 
\textbf{3.b)} \ 2nd-order forward kinematics of robot mechanism: \\ 
%TCIMACRO{\TeXButton{9ex}{\hspace{9ex}}}%
%BeginExpansion
\hspace{9ex}%
%EndExpansion
\begin{tabular}{l}
For $i=1,\ldots ,n-1$ do \\ 
%TCIMACRO{\TeXButton{2ex}{\hspace{2ex}}}%
%BeginExpansion
\hspace{2ex}%
%EndExpansion
\begin{tabular}{rl}
$\dot{\mathbf{V}}_{i}^{\text{s}}=%
%TCIMACRO{\TeXButton{-2ex}{\hspace{-2ex}}}%
%BeginExpansion
\hspace{-2ex}%
%EndExpansion
$ & $\mathbf{V}_{i-1}^{\text{s}}+\mathbf{S}_{i}\ddot{q}_{i}+\dot{\mathbf{S}}%
_{i}\dot{q}_{i}$ \\ 
$\ddot{\mathbf{S}}_{i}=%
%TCIMACRO{\TeXButton{-2ex}{\hspace{-2ex}}}%
%BeginExpansion
\hspace{-2ex}%
%EndExpansion
$ & $%
%TCIMACRO{\TeXButton{big}{\big}}%
%BeginExpansion
\big%
%EndExpansion
(\mathbf{ad}_{\dot{\mathbf{V}}_{i}^{\text{s}}}+\mathbf{ad}_{\mathbf{V}_{i}^{%
\text{s}}}^{2}%
%TCIMACRO{\TeXButton{big}{\big}}%
%BeginExpansion
\big%
%EndExpansion
)\mathbf{S}_{i}$%
\end{tabular}
\\ 
End%
\end{tabular}
\\ 
\textbf{4.a)} \ 3rd-order inverse kinematics of manipulator: \\ 
%TCIMACRO{\TeXButton{10ex}{\hspace{10ex}}}%
%BeginExpansion
\hspace{10ex}%
%EndExpansion
$\dddot{\mathbf{q}}=\mathbf{J}^{-1}%
%TCIMACRO{\TeXButton{Big}{\Big}}%
%BeginExpansion
\Big%
%EndExpansion
(\ddot{\mathbf{V}}_{\mathrm{E}}^{\text{s}}-\sum_{i\leq n}(2\dot{\mathbf{S}}%
_{i}\ddot{q}_{i}+\ddot{\mathbf{S}}_{i}\dot{q}_{i})%
%TCIMACRO{\TeXButton{Big}{\Big}}%
%BeginExpansion
\Big%
%EndExpansion
)$ \\ 
\textbf{4.b)} \ 3rd-order forward kinematics of robot mechanism: \\ 
%TCIMACRO{\TeXButton{1ex}{\hspace{1ex}}}%
%BeginExpansion
\hspace{1ex}%
%EndExpansion
\begin{tabular}{l}
For $i=1,\ldots ,n-1$ do \\ 
%TCIMACRO{\TeXButton{1ex}{\hspace{1ex}}}%
%BeginExpansion
\hspace{1ex}%
%EndExpansion
\begin{tabular}{rl}
$\ddot{\mathbf{V}}_{i}^{\text{s}}=%
%TCIMACRO{\TeXButton{-2ex}{\hspace{-2ex}}}%
%BeginExpansion
\hspace{-2ex}%
%EndExpansion
$ & $\ddot{\mathbf{V}}_{i-1}^{\text{s}}+\mathbf{S}_{i}\dddot{q}_{i}+2\dot{%
\mathbf{S}}_{i}\ddot{q}_{i}+\ddot{\mathbf{S}}_{i}\dot{q}_{i}$ \\ 
$\dddot{\mathbf{S}}_{i}=%
%TCIMACRO{\TeXButton{-2ex}{\hspace{-2ex}}}%
%BeginExpansion
\hspace{-2ex}%
%EndExpansion
$ & $%
%TCIMACRO{\TeXButton{big}{\big}}%
%BeginExpansion
\big%
%EndExpansion
(\mathbf{ad}_{\ddot{\mathbf{V}}_{i}^{\text{s}}}+2\mathbf{ad}_{\dot{\mathbf{V}%
}_{i}^{\text{s}}}\mathbf{ad}_{\mathbf{V}_{i}^{\text{s}}}+\mathbf{ad}_{%
\mathbf{V}_{i}^{\text{s}}}\mathbf{ad}_{\dot{\mathbf{V}}_{i}^{\text{s}}}+%
\mathbf{ad}_{\mathbf{V}_{i}^{\text{s}}}^{3}%
%TCIMACRO{\TeXButton{big}{\big}}%
%BeginExpansion
\big%
%EndExpansion
)\mathbf{S}_{i}$%
\end{tabular}
\\ 
End%
\end{tabular}
\\ 
\textbf{5.a)} \ 4th-order inverse kinematics of manipulator: \\ 
$\ddot{\ddot{\mathbf{q}}}=\mathbf{J}^{-1}%
%TCIMACRO{\TeXButton{Big}{\Big}}%
%BeginExpansion
\Big%
%EndExpansion
(\dddot{\mathbf{V}}_{n}^{\text{s}}-\sum_{i\leq n}(\dot{\mathbf{S}}_{i}\dddot{%
q}_{i}+3\ddot{\mathbf{S}}_{i}\ddot{q}_{i}+\dddot{\mathbf{S}}_{i}\dot{q}_{i})%
%TCIMACRO{\TeXButton{Big}{\Big}}%
%BeginExpansion
\Big%
%EndExpansion
)$ \\ 
%TCIMACRO{\TeXButton{4ex}{\hspace{4ex}} }%
%BeginExpansion
\hspace{4ex}
%EndExpansion
\\ 
\textbf{5.b)} \ 4th-order forward kinematics of robot mechanism: \\ 
\begin{tabular}{l}
For $i=1,\ldots ,n-1$ do \\ 
%TCIMACRO{\TeXButton{2ex}{\hspace{2ex}}}%
%BeginExpansion
\hspace{2ex}%
%EndExpansion
$\dddot{\mathbf{V}}_{i}^{\text{s}}=\dddot{\mathbf{V}}_{i-1}^{\text{s}}+%
\mathbf{S}_{i}\ddot{\ddot{q}}_{i}+3\dot{\mathbf{S}}_{i}\dddot{q}_{i}+3\ddot{%
\mathbf{S}}_{i}\ddot{q}_{i}+\dddot{\mathbf{S}}_{i}\dot{q}_{i}$ \\ 
End%
\end{tabular}
\\ 
\textbf{Output:} $\dot{\mathbf{q}},\ddot{\mathbf{q}},\dddot{\mathbf{q}},%
\ddot{\ddot{\mathbf{q}}}$, $\dot{\mathbf{S}}_{i},\ddot{\mathbf{S}}_{i},%
\dddot{\mathbf{S}}_{i}$, $\mathbf{V}_{i}^{\text{s}},\dot{\mathbf{V}}_{i}^{%
\text{s}},\ddot{\mathbf{V}}_{i}^{\text{s}},\dddot{\mathbf{V}}_{i}^{\text{s}}$%
, $\mathbf{J}\left( \mathbf{q}\right) $ \\ \hline
\end{tabular}
\vspace{-3ex}
\end{figure}

==> Algorithm3.tex <==
%TCIDATA{Version=5.50.0.2960}
%TCIDATA{LaTeXparent=0,0,HighOrderInverseDyn.tex}
                      
\begin{figure}[ht]
\begin{tabular}{l}
\textbf{Algorithm 3: \red2nd-Order Inverse Dynamics Recursion}\black \\ 
\hline
\textbf{Input:} $\mathbf{C}_{i},\mathbf{V}_{i}^{\text{\textrm{s}}},\dot{%
\mathbf{V}}_{i}^{\text{\textrm{s}}},\ddot{\mathbf{V}}_{i}^{\text{\textrm{s}}%
},\dddot{\mathbf{V}}{_{i}^{\text{\textrm{s}}},}\mathbf{S}_{i},\dot{\mathbf{S}%
}_{i},\ddot{\mathbf{S}}_{i},\dddot{\mathbf{S}}_{i},i=1,\ldots ,n$ \\ 
$\ \ \ \ \ \ \ \ \ \mathbf{W}_{i}^{\mathrm{s},\mathrm{app}},\dot{\mathbf{W}}%
_{i}^{\text{\textrm{s}},\mathrm{app}},\ddot{\mathbf{W}}_{i}^{\text{\textrm{s}%
},\mathrm{app}},i=1,\ldots ,n;%
%TCIMACRO{\TeXButton{red}{\color{red}}}%
%BeginExpansion
\color{red}%
%EndExpansion
\ \dot{\mathbf{V}}_{0}^{\text{\textrm{s}}}%
%TCIMACRO{\TeXButton{black}{\color{black}}}%
%BeginExpansion
\color{black}%
%EndExpansion
$ \\ 
For $i=n,\ldots ,1$ do \\ 
\begin{tabular}{rll}
$\mathbf{M}_{i}^{\text{\textrm{s}}}%
%TCIMACRO{\TeXButton{-2ex}{\hspace{-2ex}}}%
%BeginExpansion
\hspace{-2ex}%
%EndExpansion
$ & $=%
%TCIMACRO{\TeXButton{-2ex}{\hspace{-2ex}}}%
%BeginExpansion
\hspace{-2ex}%
%EndExpansion
$ & $\mathbf{Ad}_{\mathbf{C}_{i}}^{-T}\mathbf{M}_{i}^{\text{b}}\mathbf{Ad}_{%
\mathbf{C}_{i}}^{-1}$ \\ 
$\mathbf{\Pi }_{i}^{\mathrm{s}}%
%TCIMACRO{\TeXButton{-2ex}{\hspace{-2ex}}}%
%BeginExpansion
\hspace{-2ex}%
%EndExpansion
$ & $=%
%TCIMACRO{\TeXButton{-2ex}{\hspace{-2ex}}}%
%BeginExpansion
\hspace{-2ex}%
%EndExpansion
$ & $\mathbf{M}_{i}^{\mathrm{s}}\mathbf{V}_{i}^{\mathrm{s}}$ \\ 
$\dot{\mathbf{\Pi }}{_{i}^{\mathrm{s}}}%
%TCIMACRO{\TeXButton{-2ex}{\hspace{-2ex}}}%
%BeginExpansion
\hspace{-2ex}%
%EndExpansion
$ & $=%
%TCIMACRO{\TeXButton{-2ex}{\hspace{-2ex}}}%
%BeginExpansion
\hspace{-2ex}%
%EndExpansion
$ & $\mathbf{M}_{i}^{\mathrm{s}}\dot{\mathbf{V}}_{i}^{\mathrm{s}}-\mathbf{ad}%
_{\mathbf{V}_{i}^{\mathrm{s}}}^{T}\mathbf{\Pi }_{i}^{\mathrm{s}}$ \\ 
$\ddot{\mathbf{\Pi }}{_{i}^{\mathrm{s}}}%
%TCIMACRO{\TeXButton{-2ex}{\hspace{-2ex}}}%
%BeginExpansion
\hspace{-2ex}%
%EndExpansion
$ & $=%
%TCIMACRO{\TeXButton{-2ex}{\hspace{-2ex}}}%
%BeginExpansion
\hspace{-2ex}%
%EndExpansion
$ & $\mathbf{M}_{i}^{\mathrm{s}}(\ddot{\mathbf{V}}_{i}^{\mathrm{s}}-\mathbf{%
ad}_{\mathbf{V}_{i}^{\mathrm{s}}}\dot{\mathbf{V}}_{i}^{\mathrm{s}})$ \\ 
&  & $-2\mathbf{ad}_{\mathbf{V}_{i}^{\mathrm{s}}}^{T}\dot{\mathbf{\Pi }}%
_{i}^{\mathrm{s}}-(\mathbf{ad}_{\dot{\mathbf{V}}_{i}^{\mathrm{s}}}+\mathbf{ad%
}_{\mathbf{V}_{i}^{\mathrm{s}}}^{2})^{T}\mathbf{\Pi }_{i}^{\mathrm{s}}$ \\ 
$\dddot{\mathbf{\Pi }}{_{i}^{\mathrm{s}}}%
%TCIMACRO{\TeXButton{-2ex}{\hspace{-2ex}}}%
%BeginExpansion
\hspace{-2ex}%
%EndExpansion
$ & $=%
%TCIMACRO{\TeXButton{-2ex}{\hspace{-2ex}}}%
%BeginExpansion
\hspace{-2ex}%
%EndExpansion
$ & $\mathbf{M}_{i}^{\mathrm{s}}(\dddot{\mathbf{V}}{_{i}^{\mathrm{s}}}-2%
\mathbf{ad}_{\mathbf{V}_{i}^{\mathrm{s}}}\ddot{\mathbf{V}}_{i}^{\mathrm{s}}+%
\mathbf{ad}_{\mathbf{V}_{i}^{\mathrm{s}}}^{2}\dot{\mathbf{V}}_{i}^{\mathrm{s}%
})$ \\ 
&  & $-3\mathbf{ad}_{\mathbf{V}_{i}^{\mathrm{s}}}^{T}\ddot{\mathbf{\Pi }}%
_{i}^{\mathrm{s}}-3(\mathbf{ad}_{\dot{\mathbf{V}}_{i}^{\mathrm{s}}}+\mathbf{%
ad}_{\mathbf{V}_{i}^{\mathrm{s}}}^{2})^{T}\dot{\mathbf{\Pi }}_{i}^{\mathrm{s}%
}$ \\ 
&  & $-(\mathbf{ad}_{\ddot{\mathbf{V}}_{i}^{\mathrm{s}}}+2\mathbf{ad}_{\dot{%
\mathbf{V}}_{i}^{\mathrm{s}}}\mathbf{ad}_{\mathbf{V}_{i}^{\mathrm{s}}}+%
\mathbf{ad}_{\mathbf{V}_{i}^{\mathrm{s}}}\mathbf{ad}_{\dot{\mathbf{V}}_{i}^{%
\mathrm{s}}}+\mathbf{ad}_{\mathbf{V}_{i}^{\mathrm{s}}}^{3})^{T}\mathbf{\Pi }%
_{i}^{\mathrm{s}}$ \\ 
$\bar{\mathbf{W}}_{i}^{\text{\textrm{s}}}%
%TCIMACRO{\TeXButton{-2ex}{\hspace{-2ex}}}%
%BeginExpansion
\hspace{-2ex}%
%EndExpansion
$ & $=%
%TCIMACRO{\TeXButton{-2ex}{\hspace{-2ex}}}%
%BeginExpansion
\hspace{-2ex}%
%EndExpansion
$ & $%
%TCIMACRO{\TeXButton{red}{\color{red}}}%
%BeginExpansion
\color{red}%
%EndExpansion
\bar{\mathbf{W}}_{i+1}^{\text{\textrm{s}}}+\dot{\mathbf{\Pi }}_{i}^{\mathrm{s%
}}+\bar{\mathbf{W}}_{i}^{\mathrm{s},\mathrm{app}}%
%TCIMACRO{\TeXButton{black}{\color{black}}}%
%BeginExpansion
\color{black}%
%EndExpansion
$ \\ 
$\dot{\bar{\mathbf{W}}}_{i}^{\text{\textrm{s}}}%
%TCIMACRO{\TeXButton{-2ex}{\hspace{-2ex}}}%
%BeginExpansion
\hspace{-2ex}%
%EndExpansion
$ & $=%
%TCIMACRO{\TeXButton{-2ex}{\hspace{-2ex}}}%
%BeginExpansion
\hspace{-2ex}%
%EndExpansion
$ & $%
%TCIMACRO{\TeXButton{red}{\color{red}}}%
%BeginExpansion
\color{red}%
%EndExpansion
\dot{\bar{\mathbf{W}}}_{i+1}^{\text{\textrm{s}}}+\ddot{\mathbf{\Pi }}{_{i}^{%
\mathrm{s}}}+\dot{\bar{\mathbf{W}}}_{i}^{\text{\textrm{s}},\mathrm{app}}%
%TCIMACRO{\TeXButton{black}{\color{black}}}%
%BeginExpansion
\color{black}%
%EndExpansion
$ \\ 
$\ddot{\bar{\mathbf{W}}}_{i}^{\text{\textrm{s}}}%
%TCIMACRO{\TeXButton{-2ex}{\hspace{-2ex}}}%
%BeginExpansion
\hspace{-2ex}%
%EndExpansion
$ & $=%
%TCIMACRO{\TeXButton{-2ex}{\hspace{-2ex}}}%
%BeginExpansion
\hspace{-2ex}%
%EndExpansion
$ & $%
%TCIMACRO{\TeXButton{red}{\color{red}}}%
%BeginExpansion
\color{red}%
%EndExpansion
\ddot{\bar{\mathbf{W}}}_{i+1}^{\text{\textrm{s}}}+\dddot{\mathbf{\Pi }}{%
_{i}^{\mathrm{s}}}+\ddot{\bar{\mathbf{W}}}_{i}^{\text{\textrm{s}},\mathrm{app%
}}%
%TCIMACRO{\TeXButton{black}{\color{black}}}%
%BeginExpansion
\color{black}%
%EndExpansion
$%
%TCIMACRO{\TeXButton{TeX field}{\vspace{0.5ex}} }%
%BeginExpansion
\vspace{0.5ex}
%EndExpansion
\\ 
$Q_{i}%
%TCIMACRO{\TeXButton{-2ex}{\hspace{-2ex}}}%
%BeginExpansion
\hspace{-2ex}%
%EndExpansion
$ & $=%
%TCIMACRO{\TeXButton{-2ex}{\hspace{-2ex}}}%
%BeginExpansion
\hspace{-2ex}%
%EndExpansion
$ & $\mathbf{S}_{i}^{T}\bar{\mathbf{W}}_{i}^{\text{\textrm{s}}}$ \\ 
$\dot{Q}_{i}%
%TCIMACRO{\TeXButton{-2ex}{\hspace{-2ex}}}%
%BeginExpansion
\hspace{-2ex}%
%EndExpansion
$ & $=%
%TCIMACRO{\TeXButton{-2ex}{\hspace{-2ex}}}%
%BeginExpansion
\hspace{-2ex}%
%EndExpansion
$ & $\mathbf{S}_{i}^{T}\dot{\bar{\mathbf{W}}}_{i}^{\text{\textrm{s}}}+\dot{%
\mathbf{S}}_{i}^{T}\bar{\mathbf{W}}_{i}^{\text{\textrm{s}}}$ \\ 
$\ddot{Q}_{i}%
%TCIMACRO{\TeXButton{-2ex}{\hspace{-2ex}}}%
%BeginExpansion
\hspace{-2ex}%
%EndExpansion
$ & $=%
%TCIMACRO{\TeXButton{-2ex}{\hspace{-2ex}}}%
%BeginExpansion
\hspace{-2ex}%
%EndExpansion
$ & $\mathbf{S}_{i}^{T}\ddot{\bar{\mathbf{W}}}_{i}^{\text{\textrm{s}}}+\ddot{%
\mathbf{S}}_{i}^{T}\bar{\mathbf{W}}_{i}^{\text{\textrm{s}}}+2\dot{\mathbf{S}}%
_{i}^{T}\dot{\bar{\mathbf{W}}}_{i}^{\text{\textrm{s}}}$%
\end{tabular}
\\ 
End \\ 
\textbf{Output:} $Q_{i},%
%TCIMACRO{\TeXButton{red}{\color{red}}}%
%BeginExpansion
\color{red}%
%EndExpansion
\dot{Q}_{i},\ddot{Q}_{i}%
%TCIMACRO{\TeXButton{black}{\color{black}}}%
%BeginExpansion
\color{black}%
%EndExpansion
$ and inter-body wrenches $\bar{\mathbf{W}}_{i}^{\text{\textrm{s}}},\dot{%
\bar{\mathbf{W}}}_{i}^{\text{\textrm{s}}},\ddot{\bar{\mathbf{W}}}_{i}^{\text{%
\textrm{s}}}$ \\ \hline
\end{tabular}
\end{figure}

==> abstract.tex <==
%TCIDATA{Version=5.50.0.2960}
%TCIDATA{LaTeXparent=0,0,EOM-PKM.tex}
Optimal control in general, and flatness-based control in particular, of
robotic 
%TCIMACRO{\TeXButton{red}{\color{red}}}%
%BeginExpansion
\color{red}%
%EndExpansion
arms 
%TCIMACRO{\TeXButton{black}{\color{black}} }%
%BeginExpansion
\color{black}
%EndExpansion
necessitate to compute the first and second time derivatives of the joint
torques/forces required to achieve a desired motion. In view of the required
computational efficiency, recursive $O\left( n\right) $-algorithms were
proposed to this end. Aiming at compact yet efficient formulations, a Lie
group formulation was recently proposed, making use of body-fixed and hybrid
representation of twists and wrenches. In this paper a formulation is
introduced using the spatial representation. The second-order inverse
dynamics algorithm is accompanied by a fourth-order forward and inverse
kinematics algorithm. 
%TCIMACRO{\TeXButton{red}{\color{red}}}%
%BeginExpansion
\color{red}%
%EndExpansion
An advantage of all Lie group formulations is that they can be parameterized
in terms of vectorial quantities that are readily available, rather than
using Denavit-Hartenberg parameters for instance. 
%TCIMACRO{\TeXButton{black}{\color{black}}}%
%BeginExpansion
\color{black}%
%EndExpansion
The method is demonstrated for the 7 DOF Franka Emika Panda robot.

